Character is Destiny: Can Role-Playing Language Agents Make Persona-Driven Decisions?

Can Large Language Models (LLMs) simulate humans in making important decisions? Recent research has unveiled the potential of using LLMs to develop role-playing language agents (RPLAs), mimicking mainly the knowledge and tones of various characters. However, imitative decision-making necessitates a more nuanced understanding of personas. In this paper, we benchmark the ability of LLMs in persona-driven decision-making. Specifically, we investigate whether LLMs can predict characters' decisions provided by the preceding stories in high-quality novels. Leveraging character analyses written by literary experts, we construct a dataset LIFECHOICE comprising 1,462 characters' decision points from 388 books. Then, we conduct comprehensive experiments on LIFECHOICE, with various LLMs and RPLA methodologies. The results demonstrate that state-of-the-art LLMs exhibit promising capabilities in this task, yet substantial room for improvement remains. Hence, we further propose the CHARMAP method, which adopts persona-based memory retrieval and significantly advances RPLAs on this task, achieving 5.03% increase in accuracy.

==> 050future.tex <==
Our research offers the following directions for future work:
\paragraph{Better role-playing schemes} Our work only utilizes basic role-playing methods. An important direction for future research is how to better guide the behavior and decision-making of roles through historical data.
\paragraph{Prediction of group behavior} Our work only discusses the behavior of a single role. Group behavior is more complex and requires consideration of interactions between multi-agents. Additionally, predicting group behavior can directly reconstruct corresponding scenes in books, which provides a new direction for LLM application in literature.
\paragraph{Building a dataset of real human decisions} Compared to novel data, real data may be more sparse, harder to retrieve, have a larger downstream choice space, and potentially more modes. On the other hand, constructing real human data needs to take privacy issues into account.

==> tables/data_leak.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{ccc}
\toprule
Restoration Level & \textbf{Raw input} & \textbf{Entity replacement} \\
\midrule
completely consistent & 27.5\% & 0\% \\
partially consistent & 47.5\% & 37.5\% \\
entirely different & 25.0\% & 62.5\% \\ \bottomrule
\end{tabular}
\caption{Analysis of Data Leakage Mitigation through Entity Replacement. Three restoration levels represent the model's ability to generate the original plot before and after replacement, and the percentages represent the proportions of different restoration levels.}
\label{tab:data_leak}
\end{table}


==> tables/drama.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{|l|}
    \hline
        \textbf{Query} \\
        Jaime Lannister, with the Army of the Dead invading \\
        the continent and your sister Cersei Lannister having \\ 
        other invasion plans, what will you do? \\
        \hline
        \hline
        \textbf{Description} \\
        Jaime is the eldest son of Duke Tywin Lannister and \\
        Lady Joanna of Casterly Rock... \textcolor{teal}{During his journey} \\
        \textcolor{teal}{and conversations with Brienne of Tarth, Jaime begins} \\
        \textcolor{teal}{to question his moral values and loyalties}... \textcolor{brown}{After} \\
        \textcolor{brown}{Cersei deceives him and other lords, not intending to} \\
        \textcolor{brown}{abide by the agreement against the White Walkers}... \\
        \hline
        \hline
        \textbf{Memory} \\
        \textcolor{teal}{Memory a:}“It's about loyalty.” Brienne stared at him...\\ 
        “I have to find her first. I promised Jaime. He \\
        named that sword 'Oathkeeper.' I must go to save her, \\
        succeed or die trying.” \\
        \textcolor{brown}{Memory b:}
        Ever since he was captured in the Whispering \\ 
        Wood,Jaime Lannister has not even been allowed to shave.\\
        That boy, who wanted to be Arthur Dayne when he was\\
        young, unknowingly, life took a turn, and he finally\\
        became the Smiling Knight... He mounted his warhorse\\
        heading north." \\
        \hline
    \end{tabular}
    \caption{}
    \label{tab:method}
\end{table}

% \begin{document}

% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{|l|}
%     \hline
%         \textbf{Query} \\
%         Jaime Lannister, with the Army of the Dead invading \\
%         the continent and your sister Cersei Lannister having \\
%         other invasion plans, what will you do? \\
%     \hline
%         \begin{tikzpicture}[remember picture, overlay]
%             \node[inner sep=0pt] (A) {};
%             \draw[->, thick] (A) -- ++(0,-0.8);
%         \end{tikzpicture}\\[0.8cm]
%     \hline
%         \textbf{Description} \\
%         Jaime is the eldest son of Duke Tywin Lannister and \\
%         Lady Joanna of Casterly Rock... During his journey \\
%         and conversations with Brienne of Tarth, Jaime begins \\
%         to question his moral values and loyalties... After \\
%         Cersei deceives him and other lords, not intending to \\
%         abide by the agreement against the White Walkers... \\
%     \hline
%         \begin{tikzpicture}[remember picture, overlay]
%             \node[inner sep=0pt] (B) {};
%             \draw[->, thick] (B) -- ++(0,-0.8);
%         \end{tikzpicture}\\[0.8cm]
%     \hline
%         \textbf{Memory} \\
%         “It's about loyalty.” Brienne stared at him... “I have \\
%         to find her first. I promised Jaime. He named that \\
%         sword 'Oathkeeper.' I must go to save her... \\
%         succeed or die trying.” \\
%         Ever since he was captured in the Whispering Wood,\\
%         Jaime Lannister has not even been allowed to shave.\\
%         That boy, who wanted to be Arthur Dayne when he was\\
%         young, unknowingly, life took a turn, and he finally\\
%         became the Smiling Knight... He mounted his warhorse\\
%         heading north." \\
%     \hline
%     \end{tabular}
%     \caption{}
%     \label{tab:method}
% \end{table}

% \end{document}

% \begin{figure}[h!]
% \centering
% \begin{tikzpicture}[node distance=2cm]
%   % Define the style for the boxes
%   \tikzstyle{box} = [rectangle, draw=black, thick, minimum width=3cm, minimum height=1cm, align=center]
  
%   % Draw the boxes with the content
%   \node[box] (A) {内容A};
%   \node[box] (B) [below of=A] {内容B};
%   \node[box] (C) [below of=B] {内容C};
  
%   % Draw the arrows between the boxes
%   \draw[-latex] (A) -- (B);
%   \draw[-latex] (B) -- (C);
% \end{tikzpicture}
% \caption{方框示意图}
% \label{fig:box_diagram}
% \end{figure}
